Abundances on the Main Sequence of Omega Centauri

Abundance ratios of carbon, nitrogen and strontium relative to iron, calculated using spectrum synthesis techniques, are given for a sample of main sequence and turnoff stars that belong to the globular cluster omega Centauri. The variations of carbon, nitrogen and/or strontium show several different abundance patterns as a function of [Fe/H]. The source of the enhancements/depletions in carbon, nitrogen and/or strontium may be enrichment from asymptotic giant branch stars of low (1--3 solar masses) and intermediate (3--8 solar masses) mass. Massive rotating stars which produce excess nitrogen without carbon and oxygen overabundances may also play a role. These abundances enable different contributors to be considered and incorporated into the evolutionary picture of omega Cen.

==> tab3.tex <==
\begin{deluxetable}{cccccccccrrrr}
\tabletypesize{\scriptsize}
\tablecolumns{13}
\tablewidth{0pt}
\tablenum{3}
\tablecaption{Stellar parameters, Indices and Abundances for {\wcen} sample. The full version of this table appears in the electronic version \label{tbl-3}}
\tablehead{\colhead{ID}&\colhead{V mag}&\colhead{B--V}&\colhead{Teff}&\colhead{logg}&\colhead{[Fe/H]}&\colhead{G Band}&\colhead{S3839}&\colhead{Sr}&\colhead{Ba}&\colhead{[C/Fe]}&\colhead{[N/Fe]}&\colhead{[Sr/Fe]} \\ \colhead{}&\colhead{}&\colhead{}&\colhead{}&\colhead{}&\colhead{}&\colhead{}&\colhead{}&\colhead{4077\AA}&\colhead{4554\AA}&\colhead{}&\colhead{}&\colhead{} \\ \colhead{(1)}&\colhead{(2)}&\colhead{(3)}&\colhead{(4)}&\colhead{(5)}&\colhead{(6)}&\colhead{(7)}&\colhead{(8)}&\colhead{(9)}&\colhead{(10)}&\colhead{(11)}&\colhead{(12)}&\colhead{(13)} 
}
\startdata
 1000812 & 17.470 & 0.610 &  5874 &  3.8 & --1.64 &  1.42 & --0.06 &  0.19 &  0.09 & \nodata & \nodata & \nodata \\
 1002064 & 18.290 & 0.570 &  6066 &  4.3 & --1.41 &  2.42 & --0.06 &  0.28 &  0.09 & \nodata & \nodata & \nodata \\
 1002884 & 17.490 & 0.600 &  5901 &  3.8 & --1.76 &  1.51 & --0.11 &  0.11 &  0.19 & \nodata & \nodata & \nodata \\
 1004374 & 17.500 & 0.620 &  5883 &  3.8 & --1.72 &  2.71 & --0.14 &  0.18 &  0.20 &  0.50 &  0.00 &  0.00 \\
 1005088 & 17.390 & 0.730 &  5443 &  3.6 & --1.58 &  5.79 & --0.06 &  0.18 &  0.29 & \nodata & \nodata & \nodata \\
 1005996 & 17.320 & 0.720 &  5572 &  3.7 & --1.49 &  4.95 & --0.10 &  0.37 &  0.24 & \nodata & \nodata & \nodata \\
 1006065 & 17.510 & 0.650 &  5761 &  3.8 & --1.62 &  2.48 & --0.01 &  0.11 &  0.04 & \nodata & \nodata & \nodata \\
 1006286 & 17.380 & 0.710 &  5564 &  3.7 & --1.49 &  4.64 & --0.04 &  0.29 &  0.28 & \nodata & \nodata & \nodata \\
 1006625 & 17.540 & 0.610 &  5869 &  3.8 & --1.78 &  2.07 & --0.11 &  0.06 &  0.19 & \nodata & \nodata & \nodata \\
 1006759 & 18.120 & 0.510 &  6282 &  4.2 & --1.71 &  0.73 & --0.10 &  0.07 &  0.22 & \nodata & \nodata & \nodata \\
 1006812 & 17.430 & 0.640 &  5772 &  3.8 & --1.49 &  2.71 & --0.07 &  0.07 &  0.25 & \nodata & \nodata & \nodata \\
 1006962 & 17.870 & 0.670 &  5672 &  3.9 & --1.59 &  4.43 & --0.11 &  0.41 &  0.29 &  0.40 &  0.50 &  1.40 \\
 1007266 & 18.430 & 0.530 &  6179 &  4.3 & --1.50 &  0.74 & --0.13 & --0.09 &  0.08 & \nodata & \nodata & \nodata \\
 1007362 & 17.450 & 0.680 &  5681 &  3.7 & --1.65 &  4.29 & --0.10 &  0.29 &  0.12 &  0.50 &  0.00 &  0.00 \\
 1007414 & 17.840 & 0.630 &  5869 &  3.9 & --1.44 &  2.89 & --0.13 &  0.25 &  0.27 & \nodata & \nodata & \nodata \\
\enddata 
\end{deluxetable}


==> tab6.tex <==
\begin{deluxetable}{cccccccccrrrr}
\tabletypesize{\scriptsize}
\tablecolumns{13}
\tablewidth{0pt}
\tablenum{3}
\tablecaption{Stellar parameters, Indices and Abundances for {\wcen} sample.  \label{tbl-3}}
\tablehead{\colhead{ID}&\colhead{V mag}&\colhead{B--V}&\colhead{Teff}&\colhead{logg}&\colhead{[Fe/H]}&\colhead{G Band}&\colhead{S3839}&\colhead{Sr}&\colhead{Ba}&\colhead{[C/Fe]}&\colhead{[N/Fe]}&\colhead{[Sr/Fe]} \\ \colhead{}&\colhead{}&\colhead{}&\colhead{}&\colhead{}&\colhead{}&\colhead{}&\colhead{}&\colhead{4077\AA}&\colhead{4554\AA}&\colhead{}&\colhead{}&\colhead{} \\ \colhead{(1)}&\colhead{(2)}&\colhead{(3)}&\colhead{(4)}&\colhead{(5)}&\colhead{(6)}&\colhead{(7)}&\colhead{(8)}&\colhead{(9)}&\colhead{(10)}&\colhead{(11)}&\colhead{(12)}&\colhead{(13)} }
\startdata
 1000812 & 17.470 & 0.610 &  5874 &  3.8 & --1.64 &  1.42 & --0.06 &  0.19 &  0.09 & \nodata & \nodata & \nodata \\
 1002064 & 18.290 & 0.570 &  6066 &  4.3 & --1.41 &  2.42 & --0.06 &  0.28 &  0.09 & \nodata & \nodata & \nodata \\
 1002884 & 17.490 & 0.600 &  5901 &  3.8 & --1.76 &  1.51 & --0.11 &  0.11 &  0.19 & \nodata & \nodata & \nodata \\
 1004374 & 17.500 & 0.620 &  5883 &  3.8 & --1.72 &  2.71 & --0.14 &  0.18 &  0.20 &  0.50 &  0.00 &  0.00 \\
 1005088 & 17.390 & 0.730 &  5443 &  3.6 & --1.58 &  5.79 & --0.06 &  0.18 &  0.29 & \nodata & \nodata & \nodata \\
 1005996 & 17.320 & 0.720 &  5572 &  3.7 & --1.49 &  4.95 & --0.10 &  0.37 &  0.24 & \nodata & \nodata & \nodata \\
 1006065 & 17.510 & 0.650 &  5761 &  3.8 & --1.62 &  2.48 & --0.01 &  0.11 &  0.04 & \nodata & \nodata & \nodata \\
 1006286 & 17.380 & 0.710 &  5564 &  3.7 & --1.49 &  4.64 & --0.04 &  0.29 &  0.28 & \nodata & \nodata & \nodata \\
 1006625 & 17.540 & 0.610 &  5869 &  3.8 & --1.78 &  2.07 & --0.11 &  0.06 &  0.19 & \nodata & \nodata & \nodata \\
 1006759 & 18.120 & 0.510 &  6282 &  4.2 & --1.71 &  0.73 & --0.10 &  0.07 &  0.22 & \nodata & \nodata & \nodata \\
 1006812 & 17.430 & 0.640 &  5772 &  3.8 & --1.49 &  2.71 & --0.07 &  0.07 &  0.25 & \nodata & \nodata & \nodata \\
 1006962 & 17.870 & 0.670 &  5672 &  3.9 & --1.59 &  4.43 & --0.11 &  0.41 &  0.29 &  0.40 &  0.50 &  1.40 \\
 1007266 & 18.430 & 0.530 &  6179 &  4.3 & --1.50 &  0.74 & --0.13 & --0.09 &  0.08 & \nodata & \nodata & \nodata \\
 1007362 & 17.450 & 0.680 &  5681 &  3.7 & --1.65 &  4.29 & --0.10 &  0.29 &  0.12 &  0.50 &  0.00 &  0.00 \\
 1007414 & 17.840 & 0.630 &  5869 &  3.9 & --1.44 &  2.89 & --0.13 &  0.25 &  0.27 & \nodata & \nodata & \nodata \\
 1007478 & 18.090 & 0.520 &  6260 &  4.2 & --1.64 &  1.71 & --0.06 &  0.05 &  0.07 & \nodata & \nodata & \nodata \\
 1007502 & 17.720 & 0.660 &  5804 &  3.9 & --1.33 &  2.09 &  0.05 &  0.46 &  0.28 & --0.40 &  2.00 &  0.90 \\
 1007940 & 18.250 & 0.550 &  6094 &  4.2 & --1.88 &  0.95 & --0.12 &  0.06 &  0.02 & \nodata & \nodata & \nodata \\
 1007950 & 17.350 & 0.660 &  5725 &  3.7 & --1.68 &  2.66 & --0.12 &  0.16 &  0.10 & \nodata & \nodata & \nodata \\
 1007994 & 17.730 & 0.690 &  5610 &  3.8 & --1.51 &  5.16 & --0.08 &  0.16 &  0.28 & \nodata & \nodata & \nodata \\
 1008000 & 17.550 & 0.630 &  5845 &  3.8 & --1.58 &  2.82 & --0.12 &  0.36 &  0.20 & \nodata & \nodata & \nodata \\
 1008477 & 17.670 & 0.670 &  5748 &  3.8 & --1.55 &  4.23 & --0.11 &  0.14 &  0.17 & \nodata & \nodata & \nodata \\
 1008642 & 18.500 & 0.510 &  6220 &  4.4 & --1.73 &  0.65 & --0.08 &  0.13 &  0.07 & \nodata & \nodata & \nodata \\
 1008670 & 18.530 & 0.570 &  6026 &  4.3 & --1.65 &  1.92 & --0.02 &  0.06 &  0.14 & \nodata & \nodata & \nodata \\
 1008976 & 17.420 & 0.660 &  5700 &  3.7 & --1.67 &  3.63 & --0.04 &  0.06 &  0.18 & \nodata & \nodata & \nodata \\
 1009109 & 17.900 & 0.630 &  5927 &  4.0 & --1.39 &  4.34 & --0.10 &  0.34 &  0.40 &  0.60 &  0.00 &  1.20 \\
 1009175 & 17.870 & 0.710 &  5620 &  3.9 & --1.43 &  5.41 & --0.10 &  0.46 &  0.38 &  0.50 &  0.00 &  1.00 \\
 1009189 & 17.710 & 0.680 &  5729 &  3.8 & --1.52 &  3.68 & --0.05 &  0.23 &  0.17 & \nodata & \nodata & \nodata \\
 1009312 & 17.550 & 0.640 &  5756 &  3.8 & --1.70 &  2.15 & --0.07 &  0.06 &  0.24 & \nodata & \nodata & \nodata \\
 1009633 & 18.120 & 0.530 &  6199 &  4.3 & --1.31 &  0.97 & --0.11 & --0.02 &  0.21 & \nodata & \nodata & \nodata \\
 1009665 & 17.380 & 0.680 &  5700 &  3.7 & --1.67 &  4.12 & --0.10 &  0.23 &  0.21 &  0.50 &  0.00 &  0.00 \\
 1009824 & 17.430 & 0.640 &  5793 &  3.8 & --1.56 &  2.42 & --0.07 &  0.24 &  0.22 & \nodata & \nodata & \nodata \\
 1009895 & 17.310 & 0.600 &  5984 &  3.8 & --1.13 &  2.91 & --0.14 &  0.18 &  0.24 & \nodata & \nodata & \nodata \\
 1009929 & 17.440 & 0.680 &  5669 &  3.7 & --1.55 &  3.50 & --0.10 &  0.31 &  0.19 & \nodata & \nodata & \nodata \\
 1010003 & 17.480 & 0.640 &  5855 &  3.8 & --1.62 &  2.41 & --0.06 &  0.39 &  0.06 &  0.20 &  0.00 &  1.00 \\
 1010050 & 17.490 & 0.620 &  5940 &  3.9 & --1.58 &  2.10 & --0.09 &  0.16 &  0.11 & \nodata & \nodata & \nodata \\
 1010205 & 18.120 & 0.520 &  6212 &  4.2 & --2.24 &  0.82 & --0.10 & --0.19 &  0.08 & \nodata & \nodata & \nodata \\
 1010859 & 18.530 & 0.550 &  6155 &  4.5 & --0.80 &  2.53 & --0.06 &  0.34 &  0.21 & --0.30 & \nodata & \nodata \\
 1011076 & 18.370 & 0.560 &  6067 &  4.3 & --1.40 &  1.32 &  0.00 & --0.10 &  0.24 &  0.00 &  1.50 &  0.00 \\
 1011273 & 17.410 & 0.690 &  5638 &  3.7 & --1.46 &  3.43 & --0.15 &  0.25 &  0.19 & \nodata & \nodata & \nodata \\
 1011509 & 18.230 & 0.510 &  6227 &  4.3 & --1.60 &  0.57 & --0.08 & --0.19 &  0.05 & \nodata & \nodata & \nodata \\
 1011564 & 17.940 & 0.680 &  5703 &  3.9 & --1.43 &  3.09 &  0.20 &  0.36 &  0.31 &  0.00 &  1.90 &  0.80 \\
 1011652 & 17.660 & 0.640 &  5847 &  3.9 & --1.43 &  4.79 & --0.11 &  0.33 &  0.35 &  0.70 &  0.00 &  1.00 \\
 1011793 & 18.200 & 0.510 &  6252 &  4.3 & --1.52 &  1.54 &  0.01 & --0.16 &  0.00 & \nodata & \nodata & \nodata \\
 2000917 & 18.410 & 0.550 &  6107 &  4.4 & --1.36 &  0.71 & --0.10 &  0.18 & --0.05 & \nodata & \nodata & \nodata \\
 2002022 & 18.530 & 0.560 &  6051 &  4.4 & --1.35 &  1.63 & --0.08 &  0.35 &  0.02 & \nodata & \nodata & \nodata \\
 2002637 & 17.510 & 0.640 &  5826 &  3.8 & --1.50 &  2.51 & --0.12 &  0.19 &  0.08 & \nodata & \nodata & \nodata \\
 2003541 & 17.520 & 0.650 &  5756 &  3.8 & --1.75 &  3.22 & --0.13 &  0.29 &  0.22 & \nodata & \nodata & \nodata \\
 2004666 & 17.850 & 0.600 &  5984 &  4.0 & --1.59 &  1.56 & --0.05 &  0.34 &  0.19 & \nodata & \nodata & \nodata \\
 2006400 & 17.550 & 0.650 &  5741 &  3.8 & --1.62 &  2.44 & --0.12 &  0.19 &  0.16 & \nodata & \nodata & \nodata \\
 2007141 & 17.420 & 0.640 &  5813 &  3.8 & --1.80 &  3.66 & --0.12 &  0.07 &  0.20 &  0.70 &  0.00 &  0.00 \\
 2007738 & 17.700 & 0.620 &  5880 &  3.9 & --1.68 &  2.91 & --0.12 &  0.20 &  0.19 &  0.50 &  0.00 &  0.00 \\
 2007846 & 18.460 & 0.540 &  6124 &  4.4 & --1.60 &  0.74 & --0.11 &  0.05 &  0.09 & \nodata & \nodata & \nodata \\
 2008355 & 18.070 & 0.610 &  5955 &  4.1 & --1.25 &  1.67 & --0.05 &  0.16 &  0.25 &  0.00 &  1.40 &  0.00 \\
 2009131 & 17.440 & 0.610 &  5918 &  3.8 & --1.78 &  1.74 & --0.11 &  0.09 &  0.07 & \nodata & \nodata & \nodata \\
 2009146 & 18.210 & 0.590 &  6076 &  4.3 & --0.54 &  1.51 & --0.03 &  0.21 &  0.34 & --0.70 & \nodata & \nodata \\
 2009750 & 17.750 & 0.700 &  5599 &  3.8 & --1.46 &  5.15 & --0.07 &  0.45 &  0.24 &  0.40 &  0.00 &  1.20 \\
 2010136 & 17.700 & 0.690 &  5631 &  3.8 & --1.75 &  5.88 & --0.07 &  0.31 &  0.21 &  1.00 &  0.50 &  1.00 \\
 2010637 & 17.940 & 0.610 &  5947 &  4.0 & --1.44 &  2.74 & --0.08 &  0.22 &  0.36 & \nodata & \nodata & \nodata \\
 2011805 & 17.600 & 0.640 &  5817 &  3.8 & --1.73 &  2.25 & --0.02 &  0.03 &  0.23 & \nodata & \nodata & \nodata \\
 2011906 & 17.250 & 0.700 &  5629 &  3.7 & --1.65 &  3.74 & --0.13 &  0.22 &  0.18 & \nodata & \nodata & \nodata \\
 2012538 & 18.380 & 0.540 &  6128 &  4.3 & --1.88 &  0.87 & --0.07 & --0.09 &  0.03 & \nodata & \nodata & \nodata \\
 2012616 & 18.450 & 0.530 &  6165 &  4.3 & --1.68 & --0.36 & --0.10 & --0.17 &  0.09 & \nodata & \nodata & \nodata \\
 2012908 & 17.280 & 0.700 &  5610 &  3.7 & --1.60 &  3.84 & --0.13 &  0.19 &  0.22 & \nodata & \nodata & \nodata \\
 2012970 & 18.290 & 0.530 &  6210 &  4.3 & --1.41 &  1.01 & --0.08 & --0.04 &  0.01 & \nodata & \nodata & \nodata \\
 2013040 & 18.260 & 0.540 &  6177 &  4.3 & --1.40 &  1.00 & --0.10 &  0.06 &  0.15 & \nodata & \nodata & \nodata \\
 2013190 & 18.170 & 0.520 &  6269 &  4.2 & --1.73 &  1.03 & --0.09 &  0.04 &  0.22 & \nodata & \nodata & \nodata \\
 2013453 & 17.520 & 0.690 &  5683 &  3.8 & --1.25 &  2.91 &  0.05 &  0.32 &  0.25 & --0.20 &  1.40 &  0.00 \\
 2013503 & 17.450 & 0.710 &  5622 &  3.7 & --1.36 &  3.14 &  0.04 &  0.19 &  0.21 & --0.10 &  1.30 &  0.00 \\
 2013804 & 17.810 & 0.600 &  5921 &  3.9 & --1.75 &  3.19 & --0.12 &  0.17 &  0.18 & \nodata & \nodata & \nodata \\
 2014225 & 17.790 & 0.640 &  5810 &  3.9 & --1.62 &  3.87 & --0.09 &  0.01 &  0.20 &  0.60 &  0.00 &  0.00 \\
 2014590 & 17.590 & 0.840 &  5169 &  3.6 & --1.01 &  5.17 &  0.83 &  1.27 &  0.67 & --0.40 &  2.00 &  1.00 \\
 2014741 & 17.490 & 0.650 &  5761 &  3.8 & --1.62 &  1.90 & --0.11 &  0.11 &  0.05 & \nodata & \nodata & \nodata \\
 2014869 & 17.300 & 0.730 &  5471 &  3.6 & --1.60 &  3.63 &  0.26 &  0.63 &  0.25 & --0.10 &  1.90 &  1.20 \\
 2015038 & 18.130 & 0.600 &  5970 &  4.1 & --1.49 &  2.49 & --0.13 &  0.21 &  0.26 & \nodata & \nodata & \nodata \\
 2015429 & 17.660 & 0.740 &  5497 &  3.8 & --1.51 &  3.75 &  0.14 &  0.51 &  0.21 & --0.10 &  1.60 &  0.80 \\
 2015448 & 18.220 & 0.690 &  5824 &  4.2 & --0.44 &  3.27 & --0.11 &  1.27 &  0.23 & --0.50 &  0.00 &  1.60 \\
 2015458 & 18.420 & 0.560 &  6062 &  4.4 & --1.22 &  2.24 & --0.08 &  0.01 &  0.19 & \nodata & \nodata & \nodata \\
 2015842 & 17.450 & 0.620 &  5836 &  3.8 & --1.78 &  2.09 & --0.12 &  0.12 &  0.07 & \nodata & \nodata & \nodata \\
 2015973 & 17.750 & 0.600 &  5944 &  3.9 & --1.66 &  2.69 & --0.09 &  0.12 &  0.17 & \nodata & \nodata & \nodata \\
 2016192 & 18.430 & 0.540 &  6119 &  4.3 & --1.76 &  0.73 & --0.09 &  0.00 &  0.20 & \nodata & \nodata & \nodata \\
 2016302 & 18.330 & 0.550 &  6125 &  4.3 & --1.46 &  0.67 & --0.09 & --0.09 &  0.07 & \nodata & \nodata & \nodata \\
 2016336 & 17.430 & 0.610 &  5925 &  3.8 & --1.78 &  1.62 & --0.11 &  0.00 &  0.12 & \nodata & \nodata & \nodata \\
 2016709 & 17.680 & 0.660 &  5749 &  3.8 & --1.64 &  2.13 &  0.03 &  0.37 &  0.36 &  0.00 &  1.80 &  1.00 \\
 2017000 & 17.870 & 0.600 &  5968 &  4.0 & --1.40 &  3.47 & --0.12 &  0.18 &  0.18 & \nodata & \nodata & \nodata \\
 2017338 & 17.450 & 0.640 &  5772 &  3.8 & --1.48 &  4.06 & --0.09 &  0.22 &  0.28 &  0.60 &  0.00 &  0.00 \\
 2017357 & 17.720 & 0.640 &  5824 &  3.9 & --1.34 &  2.06 & --0.04 &  0.49 &  0.15 & --0.10 &  1.60 &  0.70 \\
 2017465 & 17.790 & 0.620 &  5906 &  3.9 & --1.67 &  3.03 & --0.10 &  0.11 &  0.09 &  0.60 &  0.00 &  0.00 \\
 2017703 & 17.670 & 0.640 &  5784 &  3.8 & --1.62 &  2.84 & --0.07 &  0.28 &  0.23 &  0.10 &  1.80 &  1.00 \\
 2017905 & 17.470 & 0.620 &  5894 &  3.8 & --1.78 &  1.88 & --0.09 &  0.17 &  0.11 & \nodata & \nodata & \nodata \\
 2018037 & 17.470 & 0.610 &  5910 &  3.8 & --1.86 &  1.76 & --0.09 &  0.25 & --0.01 & \nodata & \nodata & \nodata \\
 3000553 & 18.280 & 0.490 &  6353 &  4.4 & --1.55 &  0.80 & --0.10 &  0.11 &  0.11 & \nodata & \nodata & \nodata \\
 3000799 & 18.060 & 0.490 &  6340 &  4.3 & --1.63 &  0.63 & --0.05 & --0.02 &  0.12 & \nodata & \nodata & \nodata \\
 3000929 & 17.290 & 0.720 &  5434 &  3.6 & --1.74 &  4.10 & --0.11 &  0.28 &  0.26 & \nodata & \nodata & \nodata \\
 3001362 & 17.820 & 0.630 &  5948 &  4.0 & --1.25 &  3.80 &  0.00 &  0.22 &  0.21 & \nodata & \nodata & \nodata \\
 3001426 & 17.670 & 0.830 &  5336 &  3.8 & --0.70 &  5.16 &  0.96 &  1.25 &  0.63 & --0.30 &  1.40 &  1.00 \\
 3001577 & 18.300 & 0.570 &  6059 &  4.2 & --1.50 &  1.59 & --0.07 &  0.16 &  0.11 & \nodata & \nodata & \nodata \\
 3002159 & 18.460 & 0.540 &  6122 &  4.4 & --1.65 &  0.76 & --0.05 & --0.01 &  0.22 & \nodata & \nodata & \nodata \\
 3003347 & 18.530 & 0.530 &  6182 &  4.4 & --1.54 &  1.51 & --0.10 & --0.14 &  0.11 & \nodata & \nodata & \nodata \\
 3003577 & 17.900 & 0.640 &  5836 &  4.0 & --1.43 &  4.19 & --0.14 &  0.27 &  0.32 &  0.50 &  0.00 &  0.00 \\
 3003635 & 18.390 & 0.520 &  6194 &  4.4 & --1.50 &  0.91 & --0.10 &  0.10 &  0.21 & \nodata & \nodata & \nodata \\
 3003636 & 17.440 & 0.650 &  5769 &  3.8 & --1.60 &  2.04 & --0.04 &  0.32 &  0.16 & \nodata & \nodata & \nodata \\
 3003759 & 18.430 & 0.560 &  6067 &  4.5 & --0.32 &  2.46 & --0.06 &  0.19 &  0.31 & --0.60 & \nodata & \nodata \\
 3003808 & 18.250 & 0.600 &  5968 &  4.3 & --1.00 &  2.88 & --0.14 &  0.28 &  0.16 & --0.10 & \nodata & \nodata \\
 3005301 & 18.330 & 0.600 &  5969 &  4.3 & --1.09 &  1.90 & --0.05 &  0.50 & - 0.34 &  0.00 & \nodata & \nodata \\
 3300089 & 17.960 & 0.620 &  5905 &  4.0 & --1.36 &  1.96 & --0.05 &  0.15 &  0.37 & \nodata & \nodata & \nodata \\
 3300518 & 17.660 & 0.700 &  5696 &  3.8 & --1.12 &  3.73 &  0.15 &  0.29 &  0.26 & --0.20 &  1.80 &  0.00 \\
 3300749 & 18.200 & 0.520 &  6216 &  4.3 & --1.53 &  0.82 & --0.09 & --0.01 &  0.12 & \nodata & \nodata & \nodata \\
 3300868 & 17.430 & 0.670 &  5740 &  3.8 & --1.49 &  2.97 & --0.08 &  0.13 &  0.19 & \nodata & \nodata & \nodata \\
 3301274 & 17.730 & 0.610 &  5886 &  3.9 & --1.83 &  2.05 & --0.14 &  0.01 &  0.18 & \nodata & \nodata & \nodata \\
 3301416 & 17.550 & 0.640 &  5837 &  3.8 & --1.70 &  1.53 & --0.09 &  0.20 &  0.23 & \nodata & \nodata & \nodata \\
 3301462 & 18.420 & 0.520 &  6182 &  4.3 & --1.78 &  0.69 & --0.08 &  0.24 &  0.11 & \nodata & \nodata & \nodata \\
 3301595 & 17.370 & 0.690 &  5605 &  3.7 & --1.65 &  3.57 & --0.13 &  0.27 &  0.20 & \nodata & \nodata & \nodata \\
 3302158 & 18.460 & 0.540 &  6129 &  4.3 & --1.84 &  0.77 & --0.08 &  0.02 &  0.11 & \nodata & \nodata & \nodata \\
 3302219 & 17.580 & 0.640 &  5824 &  3.8 & --1.62 &  2.43 & --0.11 &  0.25 &  0.06 & \nodata & \nodata & \nodata \\
 3302441 & 17.510 & 0.630 &  5781 &  3.8 & --1.67 &  2.37 & --0.10 &  0.21 &  0.09 & \nodata & \nodata & \nodata \\
 3302479 & 17.470 & 0.660 &  5740 &  3.8 & --1.49 &  1.78 & --0.04 &  0.27 &  0.19 & \nodata & \nodata & \nodata \\
 3303059 & 18.120 & 0.600 &  6005 &  4.1 & --1.23 &  1.73 & --0.04 &  0.36 &  0.32 & --0.30 &  1.80 &  0.00 \\
 3303238 & 18.230 & 0.610 &  5936 &  4.1 & --1.52 &  1.48 & --0.10 &  0.20 &  0.22 & \nodata & \nodata & \nodata \\
 3303294 & 17.480 & 0.660 &  5681 &  3.7 & --1.67 &  2.30 & --0.11 &  0.23 &  0.19 & \nodata & \nodata & \nodata \\
 3303663 & 18.370 & 0.530 &  6203 &  4.3 & --1.55 &  1.03 & --0.13 &  0.16 &  0.07 & \nodata & \nodata & \nodata \\
 3303724 & 18.240 & 0.530 &  6173 &  4.3 & --1.73 &  0.71 & --0.10 & --0.12 &  0.12 & \nodata & \nodata & \nodata \\
 3303974 & 18.450 & 0.620 &  5936 &  4.4 & --0.68 &  2.28 &  0.08 &  0.44 &  0.03 & --0.50 &  1.20 &  0.00 \\
 3303992 & 17.940 & 0.610 &  5950 &  4.0 & --1.50 &  2.10 & --0.08 &  0.18 &  0.17 & \nodata & \nodata & \nodata \\
 3304349 & 18.140 & 0.580 &  6066 &  4.1 & --1.25 &  1.66 &  0.03 &  0.32 &  0.23 &  0.00 &  1.70 &  0.00 \\
 3304642 & 18.030 & 0.600 &  5914 &  4.0 & --1.76 &  1.87 & --0.12 &  0.08 &  0.04 & \nodata & \nodata & \nodata \\
 3304947 & 17.720 & 0.630 &  5847 &  3.9 & --1.56 &  2.76 & --0.09 &  0.15 &  0.25 & \nodata & \nodata & \nodata \\
 3305220 & 17.570 & 0.660 &  5720 &  3.8 & --1.62 &  2.62 &  0.01 &  0.22 &  0.17 &  0.00 &  1.70 &  0.00 \\
 3305280 & 17.260 & 0.730 &  5418 &  3.6 & --1.70 &  5.52 & --0.00 &  0.27 &  0.30 & \nodata & \nodata & \nodata \\
 3305688 & 18.030 & 0.620 &  5906 &  4.0 & --1.55 &  2.82 & --0.13 &  0.30 &  0.29 &  0.20 &  0.00 &  1.20 \\
 3305795 & 18.390 & 0.580 &  6009 &  4.3 & --1.25 &  3.05 & --0.10 &  0.16 &  0.29 & \nodata & \nodata & \nodata \\
 3306079 & 17.250 & 0.680 &  5656 &  3.7 & --1.57 &  2.43 &  0.09 &  0.41 &  0.38 & --0.20 &  1.90 &  0.00 \\
 3306191 & 17.600 & 0.680 &  5681 &  3.8 & --1.49 &  3.17 &  0.03 &  0.25 &  0.14 &  0.10 &  1.40 &  0.00 \\
 3306290 & 18.250 & 0.550 &  6101 &  4.3 & --1.60 &  1.85 & --0.06 &  0.05 &  0.15 & \nodata & \nodata & \nodata \\
 3306502 & 18.210 & 0.500 &  6285 &  4.4 & --1.33 &  0.16 & --0.07 &  0.13 &  0.07 & \nodata & \nodata & \nodata \\
 3306962 & 17.630 & 0.660 &  5700 &  3.8 & --1.55 &  4.12 & --0.12 &  0.17 &  0.08 & \nodata & \nodata & \nodata \\
 3307212 & 18.120 & 0.610 &  5947 &  4.1 & --1.39 &  2.12 & --0.04 &  0.33 &  0.21 & \nodata & \nodata & \nodata \\
 4000960 & 18.190 & 0.510 &  6301 &  4.3 & --1.64 &  0.72 & --0.05 & --0.06 &  0.01 & \nodata & \nodata & \nodata \\
 4001757 & 17.940 & 0.610 &  6052 &  4.1 & --1.13 &  2.67 &  0.06 &  0.21 &  0.26 &  0.00 &  1.80 &  0.00 \\
 4002103 & 18.330 & 0.510 &  6226 &  4.3 & --1.76 &  0.59 & --0.12 & --0.07 &  0.05 & \nodata & \nodata & \nodata \\
 4002760 & 17.770 & 0.620 &  5909 &  3.9 & --1.50 &  4.20 & --0.14 &  0.29 &  0.16 &  0.60 &  0.00 &  0.00 \\
 4003446 & 18.150 & 0.580 &  6030 &  4.1 & --1.73 &  0.88 & --0.10 &  0.07 &  0.10 & \nodata & \nodata & \nodata \\
 4003468 & 18.300 & 0.530 &  6204 &  4.3 & --1.58 &  0.81 & --0.10 & --0.02 &  0.21 & \nodata & \nodata & \nodata \\
 4003473 & 17.690 & 0.680 &  5724 &  3.8 & --1.45 &  5.74 & --0.07 &  0.42 &  0.25 &  0.75 &  0.00 &  0.00 \\
 4004119 & 18.160 & 0.530 &  6182 &  4.3 & --1.67 &  1.95 & --0.11 &  0.13 &  0.24 & \nodata & \nodata & \nodata \\
 4004203 & 18.510 & 0.560 &  6073 &  4.4 & --1.38 &  2.89 & --0.10 &  0.14 &  0.18 & \nodata & \nodata & \nodata \\
 4004245 & 18.070 & 0.540 &  6167 &  4.2 & --1.71 &  1.86 & --0.09 &  0.19 &  0.24 & \nodata & \nodata & \nodata \\
 4004535 & 18.260 & 0.520 &  6207 &  4.3 & --1.50 &  0.93 & --0.15 &  0.40 &  0.06 & \nodata & \nodata & \nodata \\
 4004622 & 17.510 & 0.640 &  5845 &  3.8 & --1.62 &  2.53 & --0.13 &  0.14 &  0.09 & \nodata & \nodata & \nodata \\
 4004658 & 17.410 & 0.750 &  5399 &  3.6 & --1.42 &  4.20 &  0.51 &  0.72 &  0.45 & --0.10 &  2.00 &  1.00 \\
 4004910 & 18.250 & 0.510 &  6220 &  4.3 & --1.67 &  0.81 & --0.11 & --0.15 &  0.08 & \nodata & \nodata & \nodata \\
 4005464 & 18.460 & 0.630 &  5909 &  4.4 & --0.64 &  4.04 &  0.32 &  0.47 &  0.43 & --0.20 &  1.40 &  0.50 \\
 4005688 & 18.490 & 0.510 &  6213 &  4.4 & --1.84 &  0.22 & --0.15 &  0.52 & --0.42 & \nodata & \nodata & \nodata \\
 4005757 & 18.330 & 0.550 &  6101 &  4.3 & --1.61 &  1.56 & --0.12 &  0.16 &  0.21 & \nodata & \nodata & \nodata \\
 4006178 & 18.040 & 0.510 &  6292 &  4.2 & --1.63 &  0.95 & --0.12 &  0.00 & --0.06 & \nodata & \nodata & \nodata \\
 4006593 & 17.410 & 0.630 &  5864 &  3.8 & --1.60 &  1.97 & --0.08 &  0.21 &  0.16 & \nodata & \nodata & \nodata \\
 5001850 & 18.100 & 0.510 &  6282 &  4.2 & --1.70 &  0.90 & --0.13 &  0.11 & --1.50 & \nodata & \nodata & \nodata \\
 5002311 & 17.490 & 0.660 &  5760 &  3.8 & --1.67 &  2.67 & --0.14 &  0.07 &  0.21 & \nodata & \nodata & \nodata \\
 5002339 & 17.480 & 0.620 &  5813 &  3.8 & --1.78 &  2.25 & --0.10 & --0.03 &  0.15 & \nodata & \nodata & \nodata \\
 5002422 & 18.490 & 0.520 &  6194 &  4.4 & --1.56 &  0.39 & --0.14 & --0.10 &  0.09 & \nodata & \nodata & \nodata \\
 5002747 & 17.310 & 0.680 &  5713 &  3.7 & --1.67 &  2.96 & --0.12 &  0.32 &  0.11 & \nodata & \nodata & \nodata \\
 5002841 & 17.630 & 0.650 &  5784 &  3.8 & --1.48 &  2.56 & --0.05 &  0.17 &  0.29 &  0.10 &  1.60 &  0.00 \\
 5003039 & 18.430 & 0.540 &  6108 &  4.3 & --1.84 &  0.61 & --0.14 &  0.20 & --0.07 & \nodata & \nodata & \nodata \\
 5003151 & 17.580 & 0.740 &  5441 &  3.7 & --1.51 &  6.12 & --0.09 &  0.44 &  0.32 &  0.50 &  0.00 &  0.00 \\
 5003352 & 18.180 & 0.570 &  6058 &  4.2 & --1.54 &  1.15 & --0.09 & --0.15 &  0.13 & \nodata & \nodata & \nodata \\
 5003423 & 17.850 & 0.640 &  5869 &  3.9 & --1.46 &  2.28 &  0.03 &  0.45 &  0.19 &  0.00 &  1.80 &  1.40 \\
 5003648 & 18.270 & 0.660 &  5825 &  4.1 & --1.26 &  5.04 & --0.16 &  0.28 &  0.18 &  0.50 &  0.00 &  0.00 \\
 5003731 & 18.400 & 0.550 &  6086 &  4.4 & --1.23 &  2.20 & --0.09 &  0.80 &  0.19 & \nodata & \nodata & \nodata \\
 5003896 & 18.500 & 0.610 &  5972 &  4.3 & --0.98 &  2.41 &  0.05 &  0.16 &  0.31 & --0.40 &  1.60 &  0.00 \\
 5003964 & 18.240 & 0.570 &  6042 &  4.2 & --1.74 &  1.61 & --0.08 &  0.11 &  0.16 & \nodata & \nodata & \nodata \\
 5004458 & 18.170 & 0.640 &  5922 &  4.1 & --1.03 &  2.04 &  0.10 &  0.36 &  0.29 & --0.30 &  1.80 &  1.00 \\
 5004618 & 17.290 & 0.680 &  5647 &  3.7 & --1.69 &  3.11 & --0.10 &  0.26 &  0.09 & \nodata & \nodata & \nodata \\
 5004712 & 17.670 & 0.650 &  5765 &  3.8 & --1.55 &  2.84 & --0.13 &  0.18 &  0.08 & \nodata & \nodata & \nodata \\
 5004811 & 17.490 & 0.680 &  5702 &  3.8 & --1.40 &  2.58 &  0.04 &  0.59 &  0.13 & --0.10 &  1.70 &  1.30 \\
 5004827 & 18.300 & 0.500 &  6246 &  4.4 & --1.61 &  1.20 & --0.13 & --0.18 &  0.16 & \nodata & \nodata & \nodata \\
 5004893 & 18.380 & 0.540 &  6128 &  4.2 & --2.01 &  0.64 & --0.12 &  0.07 & --0.01 & \nodata & \nodata & \nodata \\
 5004908 & 18.090 & 0.540 &  6200 &  4.2 & --1.56 &  1.36 & --0.13 & --0.05 &  0.25 & \nodata & \nodata & \nodata \\
 5005115 & 17.550 & 0.630 &  5851 &  3.8 & --1.78 &  1.61 & --0.13 &  0.21 &  0.08 & \nodata & \nodata & \nodata \\
 5005585 & 17.530 & 0.650 &  5745 &  3.8 & --1.88 &  1.83 & --0.11 &  0.16 &  0.17 & \nodata & \nodata & \nodata \\
 5005871 & 17.910 & 0.640 &  5905 &  4.0 & --1.28 &  4.33 & --0.09 &  0.22 &  0.13 & \nodata & \nodata & \nodata \\
 5006151 & 17.540 & 0.640 &  5886 &  3.9 & --1.37 &  2.84 & --0.02 &  0.39 &  0.15 & \nodata & \nodata & \nodata \\
 5006165 & 18.140 & 0.570 &  6076 &  4.2 & --1.53 &  2.55 & --0.11 &  0.27 &  0.32 & \nodata & \nodata & \nodata \\
 5006365 & 18.340 & 0.510 &  6257 &  4.3 & --1.58 &  1.38 & --0.10 &  0.03 &  0.18 & \nodata & \nodata & \nodata \\
 5006434 & 17.500 & 0.650 &  5808 &  3.8 & --1.43 &  2.89 & --0.11 &  0.13 &  0.22 & \nodata & \nodata & \nodata \\
 5006515 & 18.220 & 0.510 &  6243 &  4.3 & --1.68 &  0.86 & --0.12 &  0.11 & --1.06 & \nodata & \nodata & \nodata \\
 5006774 & 18.520 & 0.530 &  6139 &  4.4 & --1.73 &  0.80 & --0.12 & --0.01 &  0.29 & \nodata & \nodata & \nodata \\
 5007202 & 17.830 & 0.610 &  5987 &  4.0 & --1.49 &  3.27 & --0.12 &  0.33 &  0.24 &  0.50 &  0.00 &  0.00 \\
 5007594 & 17.830 & 0.600 &  5992 &  4.0 & --1.34 &  1.75 & --0.08 &  0.37 &  0.24 & \nodata & \nodata & \nodata \\
 5007904 & 17.640 & 0.640 &  5784 &  3.8 & --1.52 &  2.36 & --0.02 &  0.28 &  0.23 & \nodata & \nodata & \nodata \\
 5008178 & 18.460 & 0.530 &  6162 &  4.4 & --1.73 &  0.28 & --0.13 & --0.11 &  0.03 & \nodata & \nodata & \nodata \\
 5008341 & 18.190 & 0.520 &  6252 &  4.3 & --1.40 &  1.01 & --0.10 &  0.02 & --0.09 & \nodata & \nodata & \nodata \\
 5008405 & 18.520 & 0.520 &  6213 &  4.4 & --1.73 &  0.89 & --0.10 & --0.05 & --0.23 & \nodata & \nodata & \nodata \\
 5010112 & 18.390 & 0.540 &  6148 &  4.3 & --1.59 &  2.35 & --0.10 &  0.12 &  0.11 & \nodata & \nodata & \nodata \\
 5010483 & 18.170 & 0.560 &  6086 &  4.2 & --1.72 &  1.57 & --0.10 &  0.25 &  0.16 & \nodata & \nodata & \nodata \\
 5011158 & 18.490 & 0.570 &  6072 &  4.4 & --1.16 &  1.58 & --0.04 &  0.30 &  0.28 & \nodata & \nodata & \nodata \\
 5011845 & 17.310 & 0.670 &  5740 &  3.7 & --1.55 &  3.11 & --0.14 &  0.20 &  0.13 & \nodata & \nodata & \nodata \\
 5012643 & 18.090 & 0.670 &  5801 &  4.0 & --1.23 &  3.17 &  0.27 &  0.36 &  0.32 &  0.00 &  1.80 &  1.00 \\
 5014257 & 17.530 & 0.640 &  5886 &  3.9 & --1.37 &  2.07 & --0.01 &  0.37 &  0.23 & \nodata & \nodata & \nodata \\
 5014309 & 18.380 & 0.530 &  6169 &  4.3 & --1.58 &  1.38 & --0.12 &  0.10 &  0.06 & \nodata & \nodata & \nodata \\
 5018984 & 17.850 & 0.660 &  5742 &  3.9 & --1.34 &  3.10 &  0.33 &  0.38 &  0.34 &  0.00 &  2.00 &  1.00 \\
 6002139 & 17.520 & 0.670 &  5661 &  3.7 & --1.59 &  2.63 & --0.07 &  0.23 &  0.21 &  0.00 &  1.10 &  0.00 \\
 6002299 & 17.560 & 0.660 &  5721 &  3.8 & --1.67 &  3.50 & --0.12 &  0.18 &  0.22 & \nodata & \nodata & \nodata \\
 6002432 & 17.720 & 0.600 &  5893 &  3.9 & --1.81 &  1.32 & --0.08 &  0.23 &  0.01 & \nodata & \nodata & \nodata \\
 6002840 & 17.460 & 0.670 &  5681 &  3.7 & --1.67 &  2.86 & --0.12 & --0.15 &  0.13 & \nodata & \nodata & \nodata \\
 6003005 & 17.590 & 0.710 &  5549 &  3.7 & --1.64 &  5.94 & --0.10 &  0.32 &  0.19 &  0.60 &  0.00 &  1.00 \\
 6003183 & 18.460 & 0.520 &  6170 &  4.3 & --2.24 &  0.70 & --0.13 & --0.12 & --1.52 & \nodata & \nodata & \nodata \\
 6003367 & 18.250 & 0.540 &  6155 &  4.3 & --1.72 &  0.72 & --0.10 & --0.01 &  0.24 & \nodata & \nodata & \nodata \\
 6004062 & 17.790 & 0.770 &  5478 &  3.8 & --1.16 &  5.97 & --0.07 &  0.77 &  0.42 & \nodata & \nodata & \nodata \\
 6004320 & 18.230 & 0.520 &  6239 &  4.2 & --1.80 &  0.48 & --0.14 & --0.10 &  0.12 & \nodata & \nodata & \nodata \\
 6004467 & 17.630 & 0.770 &  5502 &  3.8 & --1.50 &  6.60 & --0.12 &  0.34 &  0.21 &  0.60 &  0.00 &  0.00 \\
 6004742 & 18.510 & 0.560 &  6027 &  4.3 & --1.63 &  1.24 & --0.10 &  0.18 & --0.90 & \nodata & \nodata & \nodata \\
 6004884 & 18.200 & 0.540 &  6159 &  4.3 & --1.66 &  0.98 & --0.12 &  0.02 &  0.05 & \nodata & \nodata & \nodata \\
 6004974 & 18.530 & 0.560 &  6090 &  4.4 & --1.15 &  1.34 & --0.10 &  0.24 &  0.20 & \nodata & \nodata & \nodata \\
 6005044 & 18.210 & 0.620 &  5944 &  4.2 & --1.12 &  4.59 & --0.12 &  0.37 &  0.26 &  0.30 &  0.00 &  1.20 \\
 6005446 & 18.300 & 0.540 &  6159 &  4.3 & --1.49 &  1.17 & --0.03 &  0.15 & -4.65 & \nodata & \nodata & \nodata \\
 6005469 & 17.600 & 0.640 &  5817 &  3.8 & --1.75 &  1.80 & --0.04 &  0.37 &  0.21 & \nodata & \nodata & \nodata \\
 6005524 & 17.870 & 0.640 &  5855 &  3.9 & --1.50 &  4.38 & --0.14 &  0.25 &  0.22 & \nodata & \nodata & \nodata \\
 6005592 & 18.200 & 0.520 &  6220 &  4.3 & --1.73 &  0.84 & --0.11 &  0.20 &  0.07 & \nodata & \nodata & \nodata \\
 6005749 & 17.470 & 0.620 &  5818 &  3.8 & --1.73 &  1.52 & --0.11 &  0.15 &  0.09 & \nodata & \nodata & \nodata \\
 6005770 & 18.450 & 0.550 &  6066 &  4.3 & --1.65 &  0.77 & --0.14 & --0.11 &  0.20 & \nodata & \nodata & \nodata \\
 6005881 & 18.310 & 0.540 &  6135 &  4.3 & --1.69 &  1.20 & --0.11 &  0.07 & --0.06 & \nodata & \nodata & \nodata \\
 6006062 & 17.560 & 0.620 &  5851 &  3.8 & --1.78 &  2.09 & --0.15 &  0.10 &  0.10 & \nodata & \nodata & \nodata \\
 6006185 & 18.280 & 0.500 &  6288 &  4.4 & --1.62 &  0.79 & --0.11 &  0.03 &  0.01 & \nodata & \nodata & \nodata \\
 6006216 & 17.410 & 0.720 &  5616 &  3.7 & --1.27 &  3.93 &  0.16 &  0.25 &  0.31 &  0.00 &  1.40 &  0.00 \\
 6006968 & 18.440 & 0.540 &  6122 &  4.3 & --1.69 &  0.91 & --0.12 & --0.05 &  0.20 & \nodata & \nodata & \nodata \\
 6007163 & 18.260 & 0.530 &  6202 &  4.3 & --1.45 &  1.48 & --0.14 &  0.22 &  0.20 & \nodata & \nodata & \nodata \\
 6007540 & 18.080 & 0.560 &  6136 &  4.2 & --1.52 &  2.12 & --0.13 &  0.17 &  0.17 & \nodata & \nodata & \nodata \\
 6007956 & 18.470 & 0.580 &  5981 &  4.3 & --1.51 &  2.70 & --0.10 &  0.02 &  0.16 & \nodata & \nodata & \nodata \\
 6008042 & 18.160 & 0.580 &  6059 &  4.2 & --1.50 &  2.30 & --0.13 &  0.13 &  0.12 & \nodata & \nodata & \nodata \\
 6008141 & 18.320 & 0.530 &  6159 &  4.3 & --1.84 &  1.07 & --0.05 &  0.00 &  0.14 & \nodata & \nodata & \nodata \\
 6008522 & 18.450 & 0.520 &  6206 &  4.4 & --1.62 &  1.07 & --0.16 &  0.34 & --1.84 & \nodata & \nodata & \nodata \\
 6009141 & 17.670 & 0.650 &  5765 &  3.8 & --1.55 &  4.21 & --0.12 &  0.22 &  0.11 & \nodata & \nodata & \nodata \\
 6009213 & 18.500 & 0.560 &  6067 &  4.3 & --1.52 &  0.94 & --0.10 & --0.01 & --1.06 & \nodata & \nodata & \nodata \\
 6009379 & 17.530 & 0.660 &  5796 &  3.8 & --1.44 &  3.90 & --0.14 &  0.36 &  0.32 & \nodata & \nodata & \nodata \\
 6009702 & 18.500 & 0.510 &  6234 &  4.4 & --1.58 &  0.63 & --0.13 & --0.05 &  0.03 & \nodata & \nodata & \nodata \\
 6010916 & 17.320 & 0.690 &  5629 &  3.7 & --1.67 &  3.75 & --0.05 &  0.16 &  0.20 & \nodata & \nodata & \nodata \\
 6012003 & 18.320 & 0.530 &  6167 &  4.3 & --1.78 &  0.60 & --0.14 &  0.05 &  0.06 & \nodata & \nodata & \nodata \\
 6012026 & 17.360 & 0.630 &  5901 &  3.8 & --1.58 &  2.55 & --0.13 &  0.25 &  0.10 & \nodata & \nodata & \nodata \\
 6012986 & 18.510 & 0.520 &  6169 &  4.4 & --1.50 &  1.46 & --0.15 & --0.10 & --0.06 & \nodata & \nodata & \nodata \\
 6013047 & 18.200 & 0.580 &  6062 &  4.2 & --1.36 &  2.68 & --0.13 &  0.21 &  0.16 & \nodata & \nodata & \nodata \\
 6014847 & 17.600 & 0.660 &  5721 &  3.8 & --1.54 &  4.74 & --0.13 &  0.48 &  0.21 & \nodata & \nodata & \nodata \\
 6015714 & 18.260 & 0.490 &  6315 &  4.3 & --1.64 &  0.61 & --0.10 & --0.21 & --0.06 & \nodata & \nodata & \nodata \\
 6015843 & 18.200 & 0.560 &  6101 &  4.2 & --1.37 &  3.09 & --0.12 &  0.30 &  0.26 &  0.60 &  0.00 &  0.00 \\
 7000503 & 18.040 & 0.490 &  6312 &  4.3 & --1.60 &  0.62 & --0.09 & --0.11 &  0.23 & \nodata & \nodata & \nodata \\
 7001252 & 17.540 & 0.670 &  5661 &  3.7 & --1.59 &  3.57 & --0.12 &  0.30 &  0.13 & \nodata & \nodata & \nodata \\
 7001451 & 17.390 & 0.650 &  5793 &  3.8 & --1.55 &  2.95 & --0.10 &  0.28 &  0.14 & \nodata & \nodata & \nodata \\
 7001538 & 18.290 & 0.560 &  6080 &  4.2 & --1.75 &  1.80 & --0.08 &  0.08 &  0.11 & \nodata & \nodata & \nodata \\
 7001810 & 17.360 & 0.660 &  5708 &  3.7 & --1.53 &  4.00 & --0.05 &  0.33 &  0.16 & \nodata & \nodata & \nodata \\
 7002266 & 17.260 & 0.670 &  5660 &  3.7 & --1.49 &  3.48 & --0.13 &  0.20 &  0.15 & \nodata & \nodata & \nodata \\
 7002429 & 18.480 & 0.530 &  6182 &  4.4 & --1.54 &  0.65 & --0.10 &  0.18 &  0.14 & \nodata & \nodata & \nodata \\
 7002707 & 17.630 & 0.660 &  5762 &  3.8 & --1.52 &  3.70 &  0.12 &  0.42 &  0.15 &  0.20 &  1.70 &  0.80 \\
 7002710 & 17.640 & 0.640 &  5804 &  3.8 & --1.57 &  3.25 & --0.16 &  0.42 &  0.18 & \nodata & \nodata & \nodata \\
 7002981 & 18.200 & 0.490 &  6320 &  4.4 & --1.52 &  0.53 & --0.14 & --0.02 &  0.13 & \nodata & \nodata & \nodata \\
 7003200 & 17.700 & 0.640 &  5847 &  3.9 & --1.48 &  2.82 &  0.12 &  0.48 &  0.27 &  0.10 &  1.80 &  1.30 \\
 7003737 & 17.510 & 0.690 &  5683 &  3.8 & --1.25 &  5.19 & --0.15 &  0.39 &  0.24 & \nodata & \nodata & \nodata \\
 7004082 & 17.540 & 0.600 &  6006 &  3.9 & --1.34 &  1.17 & --0.10 &  0.23 &  0.35 & \nodata & \nodata & \nodata \\
 7004139 & 17.310 & 0.750 &  5365 &  3.6 & --1.49 &  5.67 & --0.08 &  0.53 &  0.35 & \nodata & \nodata & \nodata \\
 7004718 & 18.410 & 0.490 &  6311 &  4.4 & --1.52 &  0.37 & --0.14 &  0.01 &  0.25 & \nodata & \nodata & \nodata \\
 7005084 & 17.710 & 0.680 &  5695 &  3.8 & --1.28 &  5.06 & --0.11 &  0.31 &  0.27 & \nodata & \nodata & \nodata \\
 7005085 & 18.250 & 0.530 &  6166 &  4.5 & --0.42 &  2.11 & --0.10 &  0.18 &  0.12 & --0.40 & \nodata & \nodata \\
 7005530 & 18.330 & 0.480 &  6330 &  4.5 & --0.78 &  1.31 & --0.14 & --0.03 & --0.04 & --0.10 & \nodata & \nodata \\
 7006137 & 18.060 & 0.510 &  6282 &  4.2 & --1.72 &  0.84 & --0.10 & --0.01 &  0.12 & \nodata & \nodata & \nodata \\
 7006442 & 18.250 & 0.490 &  6307 &  4.4 & --1.57 &  0.48 & --0.13 & --0.14 &  0.05 & \nodata & \nodata & \nodata \\
 7006447 & 18.110 & 0.520 &  6249 &  4.3 & --1.72 &  1.09 & --0.12 &  0.00 & --0.49 & \nodata & \nodata & \nodata \\
 7006463 & 17.490 & 0.620 &  5813 &  3.8 & --1.78 &  2.16 & --0.11 &  0.28 &  0.13 & \nodata & \nodata & \nodata \\
 7006571 & 18.220 & 0.490 &  6320 &  4.4 & --1.52 &  0.61 & --0.14 &  0.21 &  0.00 & \nodata & \nodata & \nodata \\
 7006825 & 18.420 & 0.510 &  6220 &  4.4 & --1.58 &  0.32 & --0.12 &  0.17 &  0.35 & \nodata & \nodata & \nodata \\
 7007024 & 17.270 & 0.660 &  5744 &  3.7 & --1.43 &  3.30 & --0.12 &  0.14 &  0.16 & \nodata & \nodata & \nodata \\
 7007295 & 18.160 & 0.640 &  5893 &  4.1 & --1.31 &  2.11 &  0.10 &  0.57 &  0.34 &  0.00 &  1.50 &  1.30 \\
 7007334 & 18.440 & 0.530 &  6152 &  4.3 & --1.84 &  4.18 & --0.10 &  0.20 &  0.27 &  1.35 &  0.00 &  0.00 \\
 7007580 & 17.450 & 0.690 &  5638 &  3.7 & --1.46 &  4.09 & --0.08 &  0.42 &  0.19 & \nodata & \nodata & \nodata \\
 7007894 & 18.420 & 0.520 &  6157 &  4.3 & --1.78 &  0.38 & --0.12 & --0.10 &  0.00 & \nodata & \nodata & \nodata \\
 7008043 & 17.490 & 0.660 &  5808 &  3.8 & --1.43 &  3.55 & --0.13 &  0.32 &  0.19 & \nodata & \nodata & \nodata \\
 7008705 & 18.460 & 0.600 &  5951 &  4.3 & --1.13 &  3.94 & --0.11 &  0.20 &  0.30 & \nodata & \nodata & \nodata \\
 7008786 & 17.430 & 0.620 &  5891 &  3.8 & --1.72 &  2.36 & --0.12 &  0.07 &  0.27 & \nodata & \nodata & \nodata \\
 7009168 & 18.320 & 0.500 &  6299 &  4.3 & --1.68 &  0.67 & --0.09 &  0.02 &  0.11 & \nodata & \nodata & \nodata \\
 7009196 & 17.630 & 0.630 &  5861 &  3.9 & --1.38 &  1.90 & --0.03 &  0.41 &  0.15 & \nodata & \nodata & \nodata \\
 7009666 & 18.220 & 0.520 &  6212 &  4.3 & --1.33 &  1.31 & --0.13 &  0.03 &  0.05 & \nodata & \nodata & \nodata \\
 7010227 & 17.760 & 0.660 &  5917 &  4.0 & --0.82 &  5.10 & --0.12 &  0.56 &  0.50 &  0.30 &  0.00 &  0.80 \\
 7010305 & 17.890 & 0.670 &  5672 &  3.9 & --1.59 &  2.73 &  0.27 &  0.55 &  0.48 & \nodata & \nodata & \nodata \\
 7010505 & 18.030 & 0.540 &  6146 &  4.1 & --1.76 &  0.99 & --0.11 & --0.10 &  0.19 & \nodata & \nodata & \nodata \\
 7011049 & 17.800 & 0.620 &  5909 &  3.9 & --1.52 &  4.58 & --0.05 &  0.19 &  0.22 &  0.80 &  0.00 &  0.00 \\
 7011795 & 17.440 & 0.710 &  5629 &  3.7 & --1.46 &  4.86 & --0.01 &  0.33 &  0.31 &  0.40 &  1.00 &  0.00 \\
 7012444 & 18.230 & 0.520 &  6239 &  4.3 & --1.58 &  1.45 & --0.00 &  0.00 &  0.16 & \nodata & \nodata & \nodata \\
 7012601 & 17.600 & 0.610 &  5851 &  3.8 & --1.80 &  2.47 & --0.10 &  0.16 &  0.07 & \nodata & \nodata & \nodata \\
 7012808 & 17.270 & 0.710 &  5535 &  3.6 & --1.60 &  2.66 & --0.01 &  0.08 &  0.26 & \nodata & \nodata & \nodata \\
 7013214 & 17.610 & 0.680 &  5753 &  3.8 & --1.33 &  3.04 &  0.20 &  0.54 &  0.38 &  0.00 &  1.80 &  0.80 \\
 7013231 & 17.900 & 0.610 &  5950 &  4.0 & --1.49 &  3.44 & --0.13 &  0.28 &  0.21 &  0.60 &  0.00 &  1.00 \\
 7013452 & 17.280 & 0.700 &  5634 &  3.7 & --1.46 &  4.98 & --0.10 &  0.36 &  0.31 & \nodata & \nodata & \nodata \\
 7013743 & 18.030 & 0.600 &  5924 &  4.0 & --1.53 &  3.43 & --0.07 &  0.13 & --0.08 & \nodata & \nodata & \nodata \\
 7014056 & 17.720 & 0.650 &  5748 &  3.8 & --1.57 &  4.02 & --0.10 &  0.30 &  0.29 & \nodata & \nodata & \nodata \\
 7014120 & 17.740 & 0.620 &  6031 &  4.0 & --1.02 &  3.72 & --0.11 &  0.42 & - 0.15 &  0.00 & \nodata & \nodata \\
 7014148 & 18.300 & 0.520 &  6252 &  4.3 & --1.49 &  0.88 & --0.09 &  0.02 &  0.10 & \nodata & \nodata & \nodata \\
 8000116 & 18.470 & 0.500 &  6305 &  4.4 & --1.39 &  0.34 & --0.09 &  0.04 & --0.19 & \nodata & \nodata & \nodata \\
 8000439 & 18.060 & 0.520 &  6253 &  4.2 & --1.38 &  1.18 & --0.06 &  0.22 &  0.27 & \nodata & \nodata & \nodata \\
 8000906 & 18.480 & 0.580 &  5990 &  4.3 & --1.25 &  4.05 & --0.11 &  0.35 &  0.17 &  0.50 &  0.00 &  1.00 \\
 8001811 & 17.800 & 0.620 &  5910 &  3.9 & --1.55 &  4.80 & --0.02 &  0.44 &  0.09 &  0.70 &  1.20 &  1.40 \\
 8002725 & 17.440 & 0.710 &  5542 &  3.7 & --1.58 &  4.82 & --0.01 &  0.45 &  0.17 & \nodata & \nodata & \nodata \\
 8003450 & 17.900 & 0.720 &  5598 &  3.9 & --1.39 &  6.30 & --0.07 &  0.51 &  0.40 &  0.70 &  0.00 &  1.00 \\
 8003784 & 17.660 & 0.600 &  5920 &  3.9 & --1.68 &  3.20 & --0.14 & --0.06 &  0.06 & \nodata & \nodata & \nodata \\
 8003936 & 17.270 & 0.700 &  5554 &  3.6 & --1.67 &  2.82 & --0.01 &  0.10 &  0.14 & \nodata & \nodata & \nodata \\
 8004259 & 17.560 & 0.630 &  5902 &  3.9 & --1.52 &  1.83 & --0.09 &  0.11 &  0.17 & \nodata & \nodata & \nodata \\
 8004972 & 17.650 & 0.740 &  5497 &  3.8 & --1.51 &  5.85 & --0.06 &  0.37 &  0.24 &  0.50 &  0.00 &  0.00 \\
 8005575 & 17.710 & 0.650 &  5818 &  3.9 & --1.31 &  2.56 &  0.08 &  0.41 &  0.25 & --0.10 &  1.70 &  1.00 \\
 8005960 & 17.770 & 0.630 &  5910 &  3.9 & --1.36 &  3.66 & --0.08 &  0.43 &  0.11 &  0.30 &  0.00 &  1.00 \\
 8005988 & 18.170 & 0.600 &  6005 &  4.1 & --1.23 &  3.60 & --0.10 &  0.32 &  0.30 &  0.50 &  0.00 &  1.00 \\
 8006648 & 17.320 & 0.660 &  5729 &  3.7 & --1.59 &  2.22 & --0.07 &  0.16 &  0.08 & \nodata & \nodata & \nodata \\
 8006742 & 17.660 & 0.860 &  5459 &  3.8 & --1.42 &  6.91 &  0.11 &  0.76 &  0.50 &  0.65 &  0.00 &  1.20 \\
 8006833 & 18.060 & 0.720 &  5640 &  4.0 & --0.91 &  4.90 &  0.62 &  0.86 &  0.49 &  0.00 &  1.80 &  1.00 \\
 8006918 & 17.880 & 0.610 &  5968 &  4.0 & --1.52 &  2.62 &  0.02 &  0.41 &  0.18 &  0.50 &  0.00 &  1.40 \\
 8007290 & 18.190 & 0.570 &  6058 &  4.2 & --1.54 &  2.32 & --0.02 &  0.29 &  0.42 & \nodata & \nodata & \nodata \\
 8007431 & 18.300 & 0.610 &  5954 &  4.2 & --1.30 &  4.79 & --0.15 &  0.29 &  0.25 &  0.60 &  0.00 &  0.00 \\
 8007880 & 17.620 & 0.720 &  5550 &  3.7 & --1.57 &  4.59 & --0.09 &  0.61 &  0.35 &  0.30 &  0.00 &  1.40 \\
 8008123 & 18.370 & 0.550 &  6101 &  4.3 & --1.61 &  1.80 & --0.13 &  0.33 &  0.14 & \nodata & \nodata & \nodata \\
 8008499 & 17.540 & 0.660 &  5796 &  3.8 & --1.43 &  4.36 & --0.09 &  0.24 &  0.16 &  0.50 &  0.00 &  0.00 \\
 8008761 & 17.280 & 0.600 &  5917 &  3.7 & --1.76 &  1.92 & --0.12 & --0.16 &  0.17 & \nodata & \nodata & \nodata \\
 8008952 & 18.150 & 0.540 &  6162 &  4.2 & --1.75 &  1.17 & --0.10 &  0.07 &  0.19 & \nodata & \nodata & \nodata \\
 8008998 & 17.660 & 0.670 &  5762 &  3.8 & --1.49 &  4.57 & --0.10 &  0.35 &  0.27 &  0.60 &  0.00 &  0.90 \\
 8009123 & 18.280 & 0.500 &  6273 &  4.4 & --1.66 &  0.95 & --0.11 &  0.06 &  0.19 & \nodata & \nodata & \nodata \\
 8009213 & 18.500 & 0.600 &  5929 &  4.3 & --1.12 &  4.44 & --0.10 &  0.19 &  0.32 & \nodata & \nodata & \nodata \\
 8009378 & 18.180 & 0.590 &  6026 &  4.1 & --1.47 &  2.70 & --0.08 &  0.20 &  0.09 & \nodata & \nodata & \nodata \\
 8010151 & 18.110 & 0.530 &  6207 &  4.3 & --1.60 &  1.03 & --0.11 &  0.16 &  0.06 & \nodata & \nodata & \nodata \\
 8010266 & 18.340 & 0.490 &  6295 &  4.4 & --1.63 &  0.74 & --0.10 & --0.05 &  0.14 & \nodata & \nodata & \nodata \\
 8010497 & 17.400 & 0.640 &  5806 &  3.8 & --1.68 &  2.04 & --0.10 &  0.02 &  0.09 & \nodata & \nodata & \nodata \\
 8010945 & 18.520 & 0.560 &  6063 &  4.4 & --1.47 &  2.04 & --0.06 & --0.11 &  0.46 & \nodata & \nodata & \nodata \\
 8011050 & 18.300 & 0.550 &  6140 &  4.3 & --1.61 &  1.29 & --0.09 &  0.03 &  0.05 & \nodata & \nodata & \nodata \\
 8011094 & 18.140 & 0.570 &  6072 &  4.1 & --1.72 &  2.48 & --0.06 &  0.06 &  0.26 & \nodata & \nodata & \nodata \\
 8011688 & 18.210 & 0.510 &  6239 &  4.3 & --1.40 &  1.06 & --0.12 &  0.31 &  0.12 & \nodata & \nodata & \nodata \\
 8012548 & 18.260 & 0.500 &  6263 &  4.4 & --1.39 &  0.94 & --0.12 & --0.03 & --0.03 & \nodata & \nodata & \nodata \\
 8012702 & 18.510 & 0.510 &  6220 &  4.4 & --1.73 &  0.54 & --0.05 &  0.09 &  0.02 & \nodata & \nodata & \nodata \\
 8012764 & 18.180 & 0.500 &  6299 &  4.3 & --1.75 &  0.79 & --0.13 &  0.01 &  0.04 & \nodata & \nodata & \nodata \\
 8013120 & 18.220 & 0.510 &  6263 &  4.3 & --1.65 &  0.77 & --0.08 & --0.05 &  0.09 & \nodata & \nodata & \nodata \\
 8013269 & 18.460 & 0.510 &  6196 &  4.4 & --1.70 &  0.75 & --0.07 &  0.03 &  0.20 & \nodata & \nodata & \nodata \\
 8013431 & 18.030 & 0.530 &  6229 &  4.2 & --1.36 &  1.44 & --0.10 &  0.20 &  0.08 & \nodata & \nodata & \nodata \\
 8014165 & 18.290 & 0.500 &  6276 &  4.4 & --1.52 &  0.55 & --0.07 &  0.02 &  0.23 & \nodata & \nodata & \nodata \\
 8014251 & 18.420 & 0.520 &  6246 &  4.4 & --1.58 &  1.44 & --0.13 &  0.08 &  0.22 & \nodata & \nodata & \nodata \\
 8014475 & 18.050 & 0.570 &  6101 &  4.2 & --1.30 &  2.44 & --0.12 &  0.22 &  0.32 & \nodata & \nodata & \nodata \\
 8014492 & 18.140 & 0.500 &  6349 &  4.3 & --1.37 &  0.66 & --0.07 &  0.06 &  0.14 & \nodata & \nodata & \nodata \\
 8014542 & 17.480 & 0.610 &  5891 &  3.8 & --1.70 &  2.22 & --0.10 &  0.15 &  0.03 & \nodata & \nodata & \nodata \\
 8014612 & 18.250 & 0.540 &  6183 &  4.3 & --1.21 &  2.71 & --0.07 &  0.03 &  0.32 & \nodata & \nodata & \nodata \\
 8015047 & 18.460 & 0.500 &  6250 &  4.4 & --1.44 &  0.71 & --0.10 &  0.04 & --0.16 & \nodata & \nodata & \nodata \\
 8015398 & 17.420 & 0.740 &  5424 &  3.6 & --1.51 &  5.92 & --0.04 &  0.53 &  0.36 & \nodata & \nodata & \nodata \\
 8016365 & 17.540 & 0.600 &  5933 &  3.8 & --1.53 &  2.69 & --0.11 &  0.33 &  0.21 & \nodata & \nodata & \nodata \\
 8016572 & 18.030 & 0.470 &  6449 &  4.3 & --1.49 &  0.74 & --0.06 &  0.04 &  0.09 & \nodata & \nodata & \nodata \\
 9002025 & 17.700 & 0.620 &  5865 &  3.9 & --1.62 &  2.91 & --0.12 &  0.19 &  0.07 & \nodata & \nodata & \nodata \\
 9002555 & 18.260 & 0.570 &  6066 &  4.3 & --1.37 &  1.69 & --0.08 &  0.13 &  0.30 & \nodata & \nodata & \nodata \\
 9002843 & 17.560 & 0.640 &  5832 &  3.8 & --1.81 &  3.67 & --0.09 &  0.04 &  0.14 &  0.70 &  0.00 &  0.00 \\
 9003408 & 17.410 & 0.700 &  5648 &  3.7 & --1.49 &  3.44 &  0.09 &  0.28 &  0.22 &  0.00 &  1.70 &  0.00 \\
 9003506 & 18.290 & 0.540 &  6162 &  4.3 & --1.62 &  0.72 & --0.13 &  0.01 &  0.12 & \nodata & \nodata & \nodata \\
 9003979 & 17.860 & 0.610 &  5891 &  3.9 & --1.53 &  3.61 & --0.15 &  0.21 &  0.33 &  0.50 &  0.00 &  0.00 \\
 9004288 & 17.840 & 0.660 &  5824 &  3.9 & --1.30 &  6.29 & --0.11 &  0.65 &  0.32 &  0.90 &  0.00 &  0.00 \\
 9004390 & 17.460 & 0.610 &  5891 &  3.8 & --1.72 &  2.13 & --0.13 &  0.12 &  0.10 & \nodata & \nodata & \nodata \\
 9004420 & 18.330 & 0.510 &  6249 &  4.4 & --1.47 &  1.13 & --0.16 &  0.06 & --0.01 & \nodata & \nodata & \nodata \\
 9004775 & 18.170 & 0.490 &  6333 &  4.3 & --1.66 &  0.52 & --0.10 &  0.07 &  0.10 & \nodata & \nodata & \nodata \\
 9004977 & 17.850 & 0.770 &  5446 &  3.8 & --1.22 &  6.85 &  0.01 &  0.67 &  0.34 & \nodata & \nodata & \nodata \\
 9005151 & 17.500 & 0.740 &  5471 &  3.7 & --1.51 &  6.17 & --0.12 &  0.41 &  0.14 & \nodata & \nodata & \nodata \\
 9005202 & 17.610 & 0.610 &  5929 &  3.9 & --1.59 &  3.03 & --0.12 &  0.19 &  0.08 &  0.50 &  0.00 &  0.00 \\
 9005309 & 18.290 & 0.540 &  6107 &  4.3 & --1.88 &  4.45 & --0.10 &  0.05 &  0.15 &  1.30 &  0.00 &  0.00 \\
 9005354 & 17.480 & 0.660 &  5750 &  3.8 & --1.57 &  3.19 & --0.10 &  0.21 &  0.21 &  0.30 &  0.90 &  0.00 \\
 9005746 & 18.410 & 0.530 &  6189 &  4.3 & --1.70 &  1.11 & --0.13 &  0.08 & --0.01 & \nodata & \nodata & \nodata \\
 9005780 & 17.610 & 0.600 &  5984 &  3.9 & --1.47 &  3.06 & --0.08 &  0.21 &  0.28 &  0.50 &  0.00 &  0.00 \\
 9006422 & 18.100 & 0.650 &  5867 &  4.1 & --1.10 &  3.43 &  0.31 &  0.56 &  0.21 &  0.00 &  1.80 &  1.10 \\
 9006600 & 18.130 & 0.500 &  6327 &  4.3 & --1.69 &  0.49 & --0.11 &  0.06 &  0.13 & \nodata & \nodata & \nodata \\
 9007008 & 18.320 & 0.560 &  6107 &  4.3 & --1.37 &  2.51 & --0.11 & --0.01 &  0.27 & \nodata & \nodata & \nodata \\
 9007066 & 17.550 & 0.640 &  5824 &  3.8 & --1.60 &  2.43 &  0.01 &  0.45 &  0.23 &  0.00 &  2.10 &  1.00 \\
 9007782 & 18.370 & 0.520 &  6194 &  4.4 & --1.50 &  0.99 & --0.09 & --0.10 &  0.01 & \nodata & \nodata & \nodata \\
 9007901 & 18.180 & 0.500 &  6311 &  4.3 & --1.47 &  0.64 & --0.12 &  0.03 &  0.04 & \nodata & \nodata & \nodata \\
 9008225 & 17.670 & 0.610 &  5907 &  3.9 & --1.61 &  2.87 & --0.11 &  0.06 &  0.35 & \nodata & \nodata & \nodata \\
 9008443 & 17.510 & 0.600 &  5951 &  3.8 & --1.62 &  1.68 & --0.08 &  0.16 &  0.22 & \nodata & \nodata & \nodata \\
 9008456 & 18.300 & 0.550 &  6118 &  4.4 & --1.10 &  2.45 & --0.12 &  0.12 &  0.17 & --0.10 & \nodata & \nodata \\
 9008495 & 17.690 & 0.650 &  5825 &  3.9 & --1.45 &  4.10 & --0.13 &  0.34 &  0.25 & \nodata & \nodata & \nodata \\
 9008929 & 17.850 & 0.660 &  5903 &  4.0 & --1.09 &  3.15 &  0.27 &  0.43 &  0.32 &  0.00 &  1.80 &  1.00 \\
 9009088 & 17.510 & 0.620 &  5883 &  3.8 & --1.72 &  2.06 & --0.09 &  0.19 &  0.17 & \nodata & \nodata & \nodata \\
 9009568 & 18.150 & 0.510 &  6301 &  4.3 & --1.66 &  0.92 & --0.04 & --0.01 &  0.07 & \nodata & \nodata & \nodata \\
 9009977 & 18.490 & 0.520 &  6209 &  4.4 & --1.63 &  0.93 & --0.15 &  0.37 &  0.12 & \nodata & \nodata & \nodata \\
 9010640 & 17.380 & 0.640 &  5802 &  3.8 & --1.49 &  2.14 & --0.10 &  0.37 &  0.13 & \nodata & \nodata & \nodata \\
 9010673 & 17.590 & 0.640 &  5825 &  3.8 & --1.55 &  3.15 & --0.06 &  0.25 &  0.31 & \nodata & \nodata & \nodata \\
 9011604 & 17.810 & 0.630 &  5888 &  3.9 & --1.46 &  3.66 & --0.12 &  0.17 &  0.18 & \nodata & \nodata & \nodata \\
\enddata 
\end{deluxetable}

